Verifying QUIC implementations using Ivy

QUIC is a new transport protocol combining the reliability and congestion control features of TCP with the security features of TLS. One of the main challenges with QUIC is to guarantee that any of its implementation follows the IETF specification. This challenge is particularly appealing as the specification is written in textual language, and hence may contain ambiguities. In a recent work, McMillan and Zuck proposed a formal representation of part of draft-18 of the IETF specification. They also showed that this representation made it possible to efficiently generate tests to stress four implementations of QUIC. Our first contribution is to complete and extend the formal representation from draft-18 to draft-29. Our second contribution is to test seven implementations of both QUIC client and server. Our last contribution is to show that our tool can highlight ambiguities in the QUIC specification, for which we suggest paths to corrections

==> body_reviewed.tex <==
%\clearpage
\section{Introduction}

% Ivy =! solver (= mthdo)

% Intro QUIC 4-5 lignes % RFC~9000 specifies the properties that QUIC implementations \textit{must} and \textit{should} have~. The specification is written in English and contains more than 250 \textit{must}-have requirements. 

\texttt{QUIC} is a new network protocol that is intended to make the Internet faster, more secure and more flexible. It is designed to replace the entire \texttt{TCP}/\texttt{TLS}/\texttt{HTTP} stack and is built above \texttt{UDP}. \texttt{QUIC} is now widely adopted and many other applications are made compatible with the protocol. This includes, for example, \texttt{MQTT}\cite{kumar2019implementation} or \texttt{DNS}\cite{huitema-quic-dnsoquic-07}. As \texttt{QUIC} is getting deployed, ensuring that \texttt{QUIC} implementations meet the set of requirements defined by the \texttt{QUIC} specification is critical. This specification is an English text document describing the protocol. It is discussed by the Internet Engineering Task Force (IETF) and is split across several Request For Comments (RFC) documents. The main document is \texttt{RFC9000}, containing more than 250 \texttt{MUST} statements indicating properties that must be met by all implementations~\cite{rfc9000}. As RFCs lack a formal definition, they can lead to ambiguities of understanding~\cite{10.1145/3472305.3472314}.%\todo{good ref ?}%\todo{related work ?}

Several approaches have been proposed to verify that \texttt{QUIC} implementations follow the specification requirements. The most common approach, called \textit{interoperability testing}, manually generates sets of tests from the requirements and then compares \texttt{QUIC} implementations with respect to those sets. This approach has been used in the \textit{QUIC-Tracker} test suite~\cite{Piraux_2018} and the \textit{QUIC Interop Runner}~\cite{quic-interop}. Albeit such approach sounds appealing, it is limited by the capacity to manually produce interesting test suites from the requirements. Another approach \cite{10.1145/3452296.3472938} is to produce a mathematical model for the protocol and its requirements, and then use formal verification to automatically assess  correctness. This approach is sound and precise. However, as it is limited to models only, it does not guarantee that subsequent implementations fulfil the requirements.%\todo{mp: si c'est pcq les implems doivent être traduite en modèle, il faut mieux l'expliciter}  

% both \todo{Retravailler cette fin de phrase, mp: je ne comprends pas la dissociation}

In a series of recent work \cite{10.1145/3341302.3342087, mcmillan2019compositional}, the authors have proposed a trade off between the two approaches. They implemented a formal language to specify protocols requirements called Ivy. Any specification written in Ivy automatically generates various and well-distributed test cases that can be exercised on \texttt{QUIC} implementation. In their work, the authors verified several requirements of \texttt{draft-18} of the \texttt{QUIC} specification. However, many requirements were left unimplemented, e.g. the management of the transport errors by \texttt{QUIC} implementations.  %\todo{CHRIS DONNE UN EXEMPLE QUE NOUS ON PEUT FAIRE} 
%Our objective is to update and expand this contribution for \texttt{draft-29} of the protocol.

Our three contributions are summarized as follows.

$(1).$ We contribute to the formal specification of \texttt{QUIC} in Ivy by implementing a significant part of \texttt{draft-29} requirements, one of the latest versions of the \texttt{QUIC} specification. This comprises new requirements and requirements in \texttt{draft-18} the authors did not model. We also update the existing requirements to the new specification. We modify Ivy to support wider variables, i.e larger than 8 bytes, enabling the tool to explore more parts of the specification. 
    %As an example, the model was originally only able to handle 8-bytes variables while many fields of the protocol are larger. 

$(2).$    We automate the use of the resulting Ivy model. We use the generated tests against seven server implementations and seven client implementations. This demonstrates that the tool can be used beyond the four original implementations tested by the authors.

$(3).$    We discuss the results we obtained and identify different types of errors in each implementation. The diversity of the results highlights contradictions and ambiguities in the %formal
    \texttt{QUIC} specification. %That is, the english specification of the protocol is ambiguous and may be hard to formalise. 
    These findings can be used to improve the \texttt{QUIC} specification. 
    We also highlight a significant disparity in the test results and hence a difference in maturity of the protocol implementations. We provide hypothesizes of the reasons why tests failed. %\todo{mp: plutot des hypotheses non?}

%mp: Si a la suite de la grande énumération qu'on vient de faire c'est pas clair c'est qu'elle est mal écrite
%This paper being a short extended abstract, it is not possible to give all modelling details of our IVY specification of \texttt{QUIC}. The main messages that should be learned from this work are (1) we improved the Ivy model of McMillan/Zuck, (2) we tested more implementations (4 to 7) than the original work, (3) we identified ambiguities in the specification of the protocol by reasoning on its various implementations. That is, our work can help to improve the IETF specification of the protocol. 

\section{The brief overview of Ivy model for \texttt{QUIC} IETF \texttt{Draft-29}}\label{sec:ivy-model}
\label{section_2}

%\setcounter{figure}{1}
\begin{figure*}[t]
    %\hspace*{-3cm}
    \vspace{-1em}\par
    \centering
    \resizebox{0.75\textwidth}{!}{%
     \begin{ganttchart}[%Specs
     y unit title=0.5cm,
     y unit chart=1cm,
     %x unit chart=0.01cm,
     vgrid,hgrid,
     title height=1,
%     title/.style={fill=none},
     title label font=\bfseries\footnotesize,
     bar/.style={fill=blue},
     bar height=0.7,
%   progress label text={},
     group right shift=0,
     group top shift=0.7,
     group height=.3,
     group peaks width={0.2},
     inline]{1}{36}
   
    %\ganttgroup[inline=false]{}{1}{36}\\
    %(mp): colors are from https://colorbrewer2.org/#type=diverging&scheme=RdYlBu&n=5
    \ganttbar[inline, bar/.append  style={fill=blue}]{\textcolor{white}{81}}{1}{9} 
    \ganttbar[inline, bar/.append  style={fill=pgreen}]{\textcolor{black}{41}}{10}{16}
    \ganttbar[inline, bar/.append  style={fill=green}]{\textcolor{black}{41}}{17}{23}
    \ganttbar[inline, bar/.append  style={fill=orange}]{\textcolor{black}{21}}{24}{26}
    \ganttbar[inline, bar/.append  style={fill=red}]{\textcolor{white}{81}}{27}{36}         %81 => 9.5
    
    \node (a) [fill=blue,draw] at ([yshift=-12pt, xshift=10pt]current bounding box.south west){\textcolor{white}{Cannot be verified}}; %, xshift=-225pt
    \node (b) [fill=pgreen,draw,anchor=west] at ([xshift=10pt]a.west west){\textcolor{black}{Original work}}; %, xshift=-180pt
    \node (c) [fill=green,draw,anchor=west] at ([xshift=10pt]b.west west){Fully implemented}; %, xshift=-300pt
    \node (d) [fill=orange,draw,anchor=west] at ([xshift=10pt]c.west west){\textcolor{black}{Partially implemented}}; %, xshift=-75pt
    \node (e) [fill=red,draw,anchor=west] at ([xshift=10pt]d.west west){\textcolor{white}{Future work}};

\end{ganttchart}
}

\caption{Tool coverage of requirements in the \texttt{QUIC} specification}
\label{must}
%\vspace{-1em}
\end{figure*}
%\todo{CHRIS DONNE UN EXEMPLE CONCRET D'UN REQUIREMENT NON VALIDE. \\ cc:\\faut t'il un example fait Al: oui et l'exemple sur le real-time du dessus doit être changé aussi puisque nous n'arrivons pas nous même à le faire. Ne jamais critiquer un scientifique sur des choses qu'on ne fait pas nous même.  ?}

%\todo{Chris pourrais tu dire quels sont les types de requirements qu'on a pu ajouter? Je me souviens t'avoir entendu parler de "tester les gestions d'erreurs". Il nous faudrait des catégories concrètes ici.}

%\texttt{QUIC} is a multi-layers client server transport protocol. Due to space limitation and to the quality of the audience, the description of \texttt{QUIC}'s stack is postponed on reading the following article\cite{rfc9000}. 
%McMillan and Zuck offered a partial Ivy model of \texttt{draft-18} of \texttt{QUIC} \texttt{IETF} specification.  
Concretely, a formal Ivy model of the protocol is defined as a set of components/nodes linked by the relationship between their input/output. Such model represents an \textit{abstraction} of the whole specification entities. Each component represents a part or a layer of the \texttt{QUIC} stack. This includes, for example, the frame layer \textcircled{1} or the packet layer \textcircled{2} presented in Figure \ref{fig:ncm}. To monitor the execution of the protocol, we define a component capturing the incoming packets, called the \texttt{shim} \textcircled{3}. %It is represented in Figure \ref{fig:ncm} with . %, for example by tracing packets on the wire. 
%components/nodes
For each received packet, the \texttt{shim} calls the \texttt{packet\_event} action, an Ivy procedure, raising an error if a requirement is violated. The \texttt{packet\_event} action contains all the requirements directly linked to the \texttt{QUIC} packet specification. It checks, for instance, that the packet number always increases. The frames are also handled similarly with their corresponding action. In Figure \ref{fig:ncm}, we can actually see that the set of requirements is directly linked to the packet component \textcircled{2}. %The \texttt{shim} is also the interface between the network and our formal specification of QUIC.
The \texttt{shim} is also in charge of translating packets from Ivy to the network.

%\todo{mp: décrire plus ivy, avec une figure. Axel: c'est un langage, seul le principe de test peut l'être avec une figure, c'est ce que fait normalement la figure 2 qui peut être améliorée. Trop tard que pour changer plus en détails.}
%mp: ok! fig 2 peut être amélioré oui

We now briefly describe our contributions to the Ivy model of \texttt{QUIC}'s specification. Our first contribution is to update this model to \texttt{draft-29} of the protocol. This is important to validate new requirements from the specification. As an example, we adapt the \texttt{shim} to the new wire format. %This component is used by  to translate abstract packets/frames into real implementation ones. 
Our second contribution is to extend the model with additional requirements for existing and new transport parameters. As an example, the \texttt{preferred\_address} transport parameter %used in migration process 
was not entirely defined in the original work, lacking a check for forbidden migration.  We also add the transport error codes management tests. For this, we create a different model which deliberately does not follow a given \texttt{QUIC} requirement in order to generate illegal packets/frames. They will be used to check whether an implementation reacts as expected, i.e. returns a specific transport error code, when receiving these packets/frames. Testing this feature is important since one can use the error code as an indication to fall back on \texttt{TCP}. % when there are problems. 
Finally, we modify Ivy to support Connection IDs (CIDs) up to 16 bytes, increasing the domain of values that can be tested and thus the coverage of our test tool. It allows testing more implementations without modifying their source code to cope with this restriction. It allows us to relax the limitation of CIDs from exactly 8 bytes to any length up to 16 bytes.
%It also allows us to generalize some heuristic\todo{mp: précise là ou enlève cette info, c'est pas assez precis ??} used originally on Connection ID which was considered as 8 bytes all the time, now it is more flexible and can adapt to any length Connection ID up to 16 bytes. 
Due to space constraints, our Ivy specification is available online\footnote{\url{https://github.com/AnonyQUIC/QUIC-Ivy}}.%\todo{mp: Pour moi, l'utilité est faible de donner le code en entier, je suis certains que les reviewers n'iront pas la regarder. Aussi, aucun pointeur n'est donné dans cette vaste code-base}
 
In Figure \ref{must}, we estimate the coverage of requirements that can be handled with our Ivy model. We distinguish five categories. The first one contains requirements that cannot be verified because they only refer to internal state, lack of formal definition or cannot be modelled in Ivy due to the limitations of technique. The second category contains requirements defined in the original work that we updated to \texttt{draft-29}. The third category contains requirements for which we implemented a complete model in the tool. The fourth category contains requirements for which we implemented a partial model, i.e. requirements for which only a part can be verified. % features for which all the requirements cannot be fully implemented. It is because some parts in the description of these requirements cannot be verified as explained for the first category.
Finally, the last category contains requirements that we leave as future work. We will now detail how these requirements are verified. 

%\todo{Christophe, je t'ai demandé d'éviter cette terminologie de safety and liveness à au moins 4 reprises. Merci de t'y tenir, il n'y a rien de pire que de redire 20 fois la même chose}

%We leveraged the new properties we modelled to increase the number of tests from 4 to 23 for the server and from 1 to 13 tests for the client. Each test sets  weights on the distribution of the type of generated frames, add new instructions directing the generated packets and additional checks for the tested requirements. In order to increase testing coverge, we also added fuzzing to several parts of the packet generation process. It allows testing more uncovered requirements of the draft


% \begin{figure*}[t]
%     %\hspace*{-3cm}
%     \vspace{-1em}\par
%     \centering
%     \resizebox{0.70\textwidth}{!}{%
%      \begin{ganttchart}[%Specs
%      y unit title=0.5cm,
%      y unit chart=1cm,
%      %x unit chart=0.01cm,
%      vgrid,hgrid,
%      title height=1,
% %     title/.style={fill=none},
%      title label font=\bfseries\footnotesize,
%      bar/.style={fill=blue},
%      bar height=0.7,
% %   progress label text={},
%      group right shift=0,
%      group top shift=0.7,
%      group height=.3,
%      group peaks width={0.2},
%      inline]{1}{36}
   
%     %\ganttgroup[inline=false]{}{1}{36}\\
%     %(mp): colors are from https://colorbrewer2.org/#type=diverging&scheme=RdYlBu&n=5
%     \ganttbar[inline, bar/.append  style={fill=blue}]{\textcolor{white}{7}}{1}{14} 
%     \ganttbar[inline, bar/.append  style={fill=pgreen}]{\textcolor{black}{0}}{15}{15}
%     \ganttbar[inline, bar/.append  style={fill=green}]{\textcolor{black}{8}}{16}{32}
%     \ganttbar[inline, bar/.append  style={fill=orange}]{\textcolor{black}{0}}{33}{33}
%     \ganttbar[inline, bar/.append  style={fill=red}]{\textcolor{white}{2}}{34}{36}         %81 => 9.5
    
%     \node (a) [fill=blue,draw] at ([yshift=-12pt, xshift=10pt]current bounding box.south west){\textcolor{white}{Cannot be verified}}; %, xshift=-225pt
%     \node (b) [fill=pgreen,draw,anchor=west] at ([xshift=10pt]a.west west){\textcolor{black}{McMillan et al.}}; %, xshift=-180pt
%     \node (c) [fill=green,draw,anchor=west] at ([xshift=10pt]b.west west){Fully implemented}; %, xshift=-300pt
%     \node (d) [fill=orange,draw,anchor=west] at ([xshift=10pt]c.west west){\textcolor{black}{Partially implemented}}; %, xshift=-75pt
%     \node (e) [fill=red,draw,anchor=west] at ([xshift=10pt]d.west west){\textcolor{white}{Future work}};

    
% \end{ganttchart}
% }

% \caption{Tool coverage of requirements in the min\_ack\_delay QUIC extension specification}
% \label{must-ext}
% \vspace{-1em}
% \end{figure*}

\vspace*{-0.5cm}

%\setcounter{figure}{0}
\begin{figure}[H]
    \centering
    \hspace*{-0.6cm}
    \includegraphics[width =1.1\columnwidth]{images/NCM.pdf}
    \caption{The \texttt{QUIC frame component} (resp. \texttt{QUIC packet component}) randomly generates frames (resp. packets) meeting its requirements, selects some of them and transmit them to the next node.
    The \texttt{shim} is the last node: it is the interface between the abstract representation of the model and the network.
    Valid \texttt{QUIC} transmissions are generated from left to right while received transmission are verified from right to left.}
    
    %Each components is linked with the input/output. A set of related requirements is also associated. Those requirements will be used with the solver to find randomly frames and packet, in this case, that respect these requirements for those generated and received. Among these valid frames/packets for the generation, we will randomly select those that will be send on the network.} %Network-centric Compositional testing: 
    \label{fig:ncm}
\end{figure}

\vspace*{-0.7cm}



\section{On Generating Test Cases}%\todo{mp: Interesting est un jugement}
\label{section_3}

\vspace*{-0.1cm}

% Notice that our specification is not an abstract implementation of the protocol, but is instead an executable monitor that observes the behavior of all protocol nodes.

Our objective is to test various implementations of both \texttt{QUIC} server and client. This is done by generating tests, i.e., sequences of packets/frames, from the formal Ivy model of the specification. The series of tests are generated with the \textit{Network-centric Compositional Testing} \cite{mcmillan2019compositional} methodology. This approach starts from a formal representation of the requirements given in the specification, that we described in Section~\ref{sec:ivy-model}, and generates traces, i.e. sequences of packets/frames, which can be sent to implementations.
%Formal specification abstract real values of variables such as IP address, frame selection, packet selection, or packet’s number. 

The tests are distinguished by the type of frames they can generate and by the distributions of those frames. The tester can manually put weights on the different frame types to influence their distributions. The weights have a default value of 1. A higher (resp. lower) weight will increase (resp. reduce) the relative probability of the associated type of frame to be generated.
For the distributions, Ivy uses the Monte Carlo sampling method \cite{shapiro2003monte} that relies on those weights.

 We cannot decide to generate or not a type of packet since their utilization is restricted to some specific situations of the protocol execution. 

%Initially set to one, the relative probability for the frame will not be affected. When the weight is less/greater than one, it reduce/increase the relative probability to select the frame.\todo{check anglais} 

The input parameters of the test are also fixed. This includes, for example, the IP address used, the port or the transport parameters. This is also done manually albeit the process can be automated with a script.

The concretization of a test is a sequence of packets/frames that are sent to the implementation under test. The test stops when a requirement is not true (failing test), or when the connection closed as expected, i.e when all the data is successfully sent (passing test). 

%The generated frames and packets, considered as conform according to the defined specification among all of the \textit{randomly} generated ones, will be \textit{randomly} selected and sent on the wire through the \texttt{shim}.

Apart from the type of frames generated and the input parameters of the test, we can also refine the existing formal specification of \texttt{QUIC} with new requirements. By moving some of these requirements from the general model to the tests, we can have more flexibility in the tests. For example, we could fix the version of \texttt{QUIC} used directly in the based formal specification but this is not convenient when one wants to change the version in different tests. Other requirements can be used to forge illegal packets. In this case we add requirements such that the model is not conforming anymore to the \texttt{QUIC} specification. As the solver guarantees that the generated frames and packets follow these added requirements it will produce non-conform frames/packets.  % We can also add requirements 

%Figure 2 presents



%%Figure \ref{fig:ncm} presents this methodology. There, the valid frames or packets are in green while the %%invalid ones are in red. %todo{on ne dit pas the Figure mais Figure}  \todo{= comment on genere des %%packets/frames}

%In Ivy, we can thus model \texttt{QUIC} with these principles\todo{Je ne comprends pas: ici on n'explique pas le langage de modélisation mais bien ce qu'on en fait pour vérifier.} based on requirements defined in the RFC. 
%One element is selected from all the possible values, using a random choice based on a Monte Carlo sampling.

% The standard structure concerning a test is that we start from our QUIC model that we have in Ivy and which allows us to test the whole set of requirements of the specification. 

%\todo{Je ne comprends pas cette phrase. Je pensais que tout cela était sélectionné de façon aléatoire, en tout cas c'est ce qui est dit plus haut. Qu'est ce qui est fait de façon aléatoire et qu'est ce que vous faites manuellement (utiliser bien les mots manuel et aléatoire) et expliquer pourquoi vous devez refaire des choses manuellement} 

% Each test relies on our \texttt{QUIC} model and adds specific refinements related to the test itself.

\vspace*{-0.2cm}

\subsection{Example}

We illustrate this approach on an example where we generate sequences of frames and packets. As explained above, each test starts from our formal specification of \texttt{QUIC}. We first manually fix the input parameters of the test. In this case, we manually set the IP addresses and the port used during the test. The tested implementation is a server. %\todo{mp: on ne sait pas si c'est un test server ou client}

\begin{lstlisting}[style=myCustomIvyStyle]
# Tester address
parameter client_addr : ip.addr = 0x7f000001
parameter client_port : ip.port = 4987
# Tested implementation address
parameter server_addr : ip.addr = 0x7f000001
parameter server_port : ip.port = 4443        
\end{lstlisting}

Then, we choose the set of frames that will be generated and the distribution of these frames in the packets. In the following example, we decide to generate \texttt{ACK}, \texttt{STREAM}, \texttt{CRYPTO} and \texttt{PATH\_RESPONSE} frames. Then we set the relative weight for the \texttt{PATH\_RESPONSE} to five. Since this is more than one, it increases the relative probability to generate this frame. This is important since otherwise, the path validation of the migration could fail.

\begin{lstlisting}[style=myCustomIvyStyle]
# Allow generation of a frame
export frame.ack.handle
export frame.stream.handle
export frame.crypto.handle
export frame.path_response.handle
# Relative weight (all other weights = 1)
attribute frame.path_response.handle.weight = "5"
\end{lstlisting}
%

%In addition, the Ivy tool can compile a generator that produces random sequences of events that conform to the specification. At each step, the generator chooses an action at random (say, ‘protocol_action’) and builds a constraint over the action’s parameters that is true exactly when all the ‘require’ conditions hold. This can be seen as either symbolic execution [6] or a weakest precondition computation [15]

%\todo{mp: décrit textuellement ce que tu as configuré avec les exports et les poids}

%features/properties
Finally, we also add specific requirements to the generated frames and packets by refining events already present in the model (i.e \texttt{packet\_event}). A requirement is indicated in Ivy with the keyword \texttt{require} and is followed by a condition. Below, we find a simple example where we randomly generate an \texttt{Initial} packet (\texttt{packet\_event}) with an \textit{invalid} "Token" field, in this case we expect a non-zero length token (see line 8). 

\begin{lstlisting}[style=myCustomIvyStyle]
# Action already present in the model
before packet_event(src:ip,dst:ip,pkt:quic_packet){
    if _generating {  # Wrong field generation
        # Applied only on generated packet
        # [...]  new features
        require ~(pkt.token.end = 0); 
    };
    # new feature (for configuration purpose)
    require pkt.long -> pkt.pversion = 0xff00001d 
}
\end{lstlisting}

As this situation is a non-conform one, we expect to receive a \texttt{PROTOCOL\_VIOLATION} error code in a \texttt{CONNECTION\_\-CLOSE} frame. This can be modelled with the special instruction \texttt{\_finalize} that allows us to check whether some requirements are eventually fulfilled.

\begin{lstlisting}[style=myCustomIvyStyle]
export action _finalize = {
    require is_invalid_token  |  ~handshake_done;
}
\end{lstlisting}


%%In some way, a test in Ivy applied to \texttt{QUIC} can be defined as a scenario where the whole %%specification will be tested each time any kind of test is launched but with different parameters for each %%test. The parameters being the three points discussed before.\todo{explain more != between test. On %%comprend %%la diff entre les tests ?} When we want to test whether a specific features is correct or not as %%for the transport error codes management, we need to create one of such test in order verify these specific %%properties. However, a scenario does not remove any requirement check and a test will be considered as %%failed as soon as one requirement in the whole specification is considered as failed. More information %%about Ivy and its concepts can be found in \cite{ivy_lang, 10.1145/3341302.3342087, %%TowardsverificationofQUICextensions}. %Some of the tests are \textit{generic}.


We will now give some details on tests made to stress the implementations  of the server and the client. Observe that the main reason to make a distinction between those two entities is that some parameters of the client and of the server are incompatible. As an example, the \texttt{preferred\_\-address} transport parameter is only available at the server side. Moreover, the generation of some frame such as the \texttt{HANDSHAK\-E\_DONE} is forbidden to the client. 

%The tests are made by adding new requirements to the generated frames and packets and is considered as failed as soon as one requirement of the whole model is not respected. Note we allow generating scenarios influencing the packet generation distribution and thus the tested properties. However, a scenario does not remove any requirement check. 


%\todo{les paraggraphes suivants sont une redite de ce qui est dit avant. Avoir une structure spec + Requirement -> test et expliquer que certains paramètres sont à fuzzer. Fait toi aider de Tom pour l'anglais}Our tests follow the methodology proposed by McMillan et al. in \cite{10.1145/3341302.3342087}. 

%This is for example, with the stream test, we test the complete specification and include the generation of valid \texttt{STREAM} frame. Other tests are \textit{more specific} in the sens that we expect a specific event to happen. A typical example is with the \textit{error} tests. There, we generate a packet that should trigger an error in the tested implementation. 

%In each type of test, all the requirements from the specification that we implemented are checked. If one requirement is not met, we report it. Note that the original work of  McMillan et al. only considers of the \textit{generic} classification. \todo{not clear ?}

%\subsection{Example}


%in addition to the standard \texttt{QUIC} model, we add some specific requirements on the different entities generated (i.e packets, frames). 

%Here is a simple example of \textit{fuzzing} where we randomly generate an \texttt{Initial} packet with an \textit{invalid} (according to the draft) "Token" field, in this case we expect a non-zero length token (see line 5). We achieve that by refining the \texttt{packet\_event} action already present in the original QUIC specification with new requirements that are applied only to the generated packets:


% \begin{lstlisting}[style=myCustomIvyStyle]
% before packet_event(src:ip,dst:ip,
%                     pkt:quic_packet) {
%     if _generating { # Wrong field generation
%         # [...]
%         require ~(pkt.token.end = 0); 
%     };
%     require pkt.long -> pkt.pversion = 0xff00001d 
% }
% \end{lstlisting}

% Since this situation is non-conform, we expect to receive a \texttt{PROTOCOL\_VIOLATION} error code in a \texttt{CONNECTION\_CLOSE} frame. We can model that in the special instruction \texttt{\_finalize} that allows to check at the end of the test where some requirements are fulfilled or not:

% \begin{lstlisting}[style=myCustomIvyStyle]
% export action _finalize = {
%     require is_invalid_token  
%         |  ~handshake_done_send;
% }
% \end{lstlisting}

% The test is considered as failed as soon as one requirement of the whole specification is not satisfied.

%\todo{Avant de commencer la section, on devrait dire pourquoi on fait un } 
%non c'est pour dire pourquoi on distingue le serveur du client, et comment on abstrait l'autre côté. 

\vspace*{-0.2cm}

\subsection{On testing server implementations}
\label{server_impl_test}


% 

% Serverquoi on fait un ter testtest servmment on abstraieur st client et coet pous

%\todo[]{faire un seul example et mettre le reste en annexe}

We have generated 23 tests to stress seven implementations of \texttt{QUIC} servers. Some of those tests are briefly described in Table \ref{tab:my-table}. 



%\vspace*{-0.3cm}

%\newpage

\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|l|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_stream}}}                                                      \\
\textbf{\begin{tabular}[c]{@{}l@{}}Generated\\ frames:\end{tabular}} & \begin{tabular}[c]{@{}l@{}}STREAM, ACK, PATH\_RESPONSE, CRYPTO\end{tabular}          \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Expected \\ output:\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Simple test where we send request to index.html. Stop once all \\ expected data is received. No error is expected.\\ Note that we allow multiple connection migrations to test its \\support as well. Several streams are open to test the streams \\mechanics. We create bidirectional streams.\end{tabular} \\
\multicolumn{2}{|l|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_unkown}}}                                                      \\
\textbf{\begin{tabular}[c]{@{}l@{}}Generated\\ frames:\end{tabular}} & \begin{tabular}[c]{@{}l@{}}STREAM, ACK, PATH\_RESPONSE, CRYPTO, UNKNOWN\end{tabular} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Expected \\ output:\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Verifies handling of UNKNOWN frame type by the implementation.\\ Only allowed in application encryption level. We expect to receive\\ a FRAME\_ENCODING\_ERROR\end{tabular} \\ \hline
 \end{tabular}%
}
%\caption{Examples of server tests}
\label{tab:my-table}
\end{table} 

\newpage

 \begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|l|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_unkown\_tp}}}                                                      \\
\textbf{\begin{tabular}[c]{@{}l@{}}Generated\\ frames:\end{tabular}} & \begin{tabular}[c]{@{}l@{}}STREAM, ACK, PATH\_RESPONSE, CRYPTO\end{tabular}          \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Expected \\ output:\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Verifies handling of UNKNOWN transport parameter by the \\ implementation.We expect the implementation to ignore the\\  transport parameter and 
  continue the execution of the protocol \\normally.\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Examples of Server Tests}
\label{tab:my-table}
\end{table}

\vspace*{-0.5cm}

Let us illustrate the approach on the \texttt{quic\_server\_te\-st\_stream} test. In this test, we generate \texttt{STREAM} frames until the number of requests is reached or until the maximal data defined during the handshake is exceeded.   Each time a generation or reception of a packet occurs, the whole specification will be tested. Moreover, as soon as one of the requirements is not satisfied, the test fails. %\todo{parler de migration multiple autorisé ? and de bidirectional stream ? Ok si dans la table 1}





% will be defined by the random process but satisfying the requirements associated
%TODO

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[H]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|ll|}
% \hline
% \multicolumn{2}{|l|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_stream}}}                                                      \\
% \textbf{\begin{tabular}[c]{@{}l@{}}Generated\\ frames:\end{tabular}} & \begin{tabular}[c]{@{}l@{}}STREAM, ACK, PATH\_RESPONSE,\\ CRYPTO\end{tabular}          \\
% \textbf{\begin{tabular}[c]{@{}l@{}}Expected \\ output:\end{tabular}} &
%   \begin{tabular}[c]{@{}l@{}}Simple test where we send request to index.html. Stop once all \\ expected data is received. No error is expected\end{tabular} \\
% \multicolumn{2}{|l|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_stream}}}                                                      \\
% \textbf{\begin{tabular}[c]{@{}l@{}}Generated\\ frames:\end{tabular}} & \begin{tabular}[c]{@{}l@{}}STREAM, ACK, PATH\_RESPONSE,\\ CRYPTO, UNKNOWN\end{tabular} \\
% \textbf{\begin{tabular}[c]{@{}l@{}}Expected \\ output:\end{tabular}} &
%   \begin{tabular}[c]{@{}l@{}}Verifies handling of UNKNOWN frame type by the implementation.\\ Only allowed in application encryption level. We expect to receive\\ a FRAME\_ENCODING\_ERROR\end{tabular} \\
% \multicolumn{2}{|l|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_stream}}}                                                      \\
% \textbf{\begin{tabular}[c]{@{}l@{}}Generated\\ frames:\end{tabular}} & \begin{tabular}[c]{@{}l@{}}STREAM, ACK, PATH\_RESPONSE,\\ CRYPTO\end{tabular}          \\
% \textbf{\begin{tabular}[c]{@{}l@{}}Expected \\ output:\end{tabular}} &
%   \begin{tabular}[c]{@{}l@{}}Verifies handling of UNKNOWN transport parameter by the \\ implementation. We expect to receive a \\ FRAME\_ENCODING\_ERROR during the handshake.\end{tabular} \\ \hline
% \end{tabular}%
% }
% \caption{Examples of server tests}
% \label{tab:my-table}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% \begin{table}[H]
% \centering
% \scriptsize
% \resizebox{\columnwidth}{!}{%

% \begin{tabular}{|l|}
% \hline
% \rowcolor[HTML]{333333} 
% {\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_stream}}                                                                                                   \\ \hline
% \begin{tabular}[c]{@{}l@{}}Verifies the full requirements and generates STREAM, ACK, \\PATH\_RESPONSE and CRYPTO frames and may perform connection \\migrations\end{tabular}             \\ 
% \hline
% \rowcolor[HTML]{333333} 
% {\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_unkown}}     \\ \hline
% \begin{tabular}[c]{@{}l@{}}Verifies handling of UNKNOWN frame type by the implementation.  \\Only allowed in  application encryption level so we must get  a \\FRAME\_ENCODING\_ERROR.\end{tabular} \\ \hline
% % \end{tabular}%
% % }
% % %\caption{Examples of server tests}
% % \label{tab:original}
% % \end{table}

% % \begin{table}[H]
% % \centering
% % \scriptsize
% % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{|l|}
% % \hline
% \rowcolor[HTML]{333333} 
% {\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_unkown\_tp}} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Verifies handling of UNKNOWN transport parameter by the implementation.\\ Must ignore it and continue execution. We disable migration in this case.\end{tabular} \\ \hline

% % \hline
% % \rowcolor[HTML]{333333} 
% % {\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_max}}                                                                                                      \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Verifies all implemented requirements and generates STREAM. Also MAX\_\\ STREAM\_DATA,  STREAM\_DATA\_BLOCKED and MAX\_DATA frames\\  with limited range field values.\end{tabular} \\ \hline
% % \rowcolor[HTML]{333333} 
% % {\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_reset\_stream}}                                                                                            \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Verifies all implemented requirements and generates STREAM and RESET\_\\ STREAM frames with random error codes.\end{tabular}     \\ \hline
% % \rowcolor[HTML]{333333} 
% % {\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_connection\_close}}                                                                                        \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Verifies all implemented requirements and generates STREAM and \\ CONNECTION\_CLOSE frames with random error codes.\end{tabular} \\ \hline
% \end{tabular}%
% }
% \caption{Examples of server tests}
% \label{tab:original}
% \end{table}

%\newpage


\subsection{On testing client implementations}

We offer 14 tests to stress seven clients’ implementations. Most of those tests are like their server counterpart. Due to space limitations, we only detail in Table \ref{tab:violation-draft} the following two errors handling tests that are specific to the client's implementation. 

For the first test, we set the "Length" field of the token to zero, which is not allowed by the draft. For the second one, we verify that the \texttt{preferred\_address} transport parameter contains zero-length connection ID and the tested implementation throws a \texttt{TRANSPORT\_PARAMETER\_ERROR}. 

It is worth mentioning that we do not perform connection migration. Indeed, such migration is triggered by the client. Testing such feature would force us to change manually the tested implementation, which would not be natural. 

%\vspace*{-0.3cm}

% \begin{table}[H]
% \centering
% \scriptsize
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|}
% \hline
% \rowcolor[HTML]{333333} 
% {\color[HTML]{FFFFFF} \textbf{quic\_client\_test\_new\_token\_error}}                                                                                            \\ \hline
% \begin{tabular}[c]{@{}l@{}}Generation of NEW\_TOKEN frames with length field set to 0. Must have\\ a PROTOCOL\_VIOLATION.\end{tabular}                         \\ %\hline
% \hline
% \rowcolor[HTML]{333333} 
% {\color[HTML]{FFFFFF} \textbf{quic\_client\_test\_prefadd\_error}} \\
% \begin{tabular}[c]{@{}l@{}}Zero length CID for preferred\_address transport parameter. \\Must have TRANSPORT\_PARAMETER\_ERROR.\end{tabular} \\ \hline
% % \rowcolor[HTML]{333333} 
% % {\color[HTML]{FFFFFF} \textbf{quic\_server\_test\_handshake\_done\_error}} \\ \hline
% % \begin{tabular}[c]{@{}l@{}}Generation of HANDSHAKE\_DONE frames before the handshake complete.\\Must have a PROTOCOL\_VIOLATION.\end{tabular} \\ \hline
% \end{tabular}%
% }
% \caption{Client specific tests}
% \label{tab:violation-draft}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[H]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ll|}
\hline
\multicolumn{2}{|l|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{quic\_client\_test\_new\_token\_error}}}     \\
\textbf{\begin{tabular}[c]{@{}l@{}}Generated\\ frames:\end{tabular}} & STREAM, ACK, HANDSHAKE\_DONE, CRYPTO, NEW\_TOKEN \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Expected \\ output:\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}We generate of NEW\_TOKEN frames with length field set to 0 \\ and expect to receive a PROTOCOL\_VIOLATION transport error.\end{tabular} \\
\multicolumn{2}{|l|}{\cellcolor[HTML]{333333}{\color[HTML]{FFFFFF} \textbf{quic\_client\_test\_prefadd\_error}}}        \\
\textbf{\begin{tabular}[c]{@{}l@{}}Generated\\ frames:\end{tabular}} & STREAM, ACK, HANDSHAKE\_DONE, CRYPTO            \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Expected \\ output:\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}We send the preferred\_address transport parameter with a zero length \\ CID field and we expect to receive a   \\TRANSPORT\_PARAMETER\_ERROR.\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Client specific tests}
\label{tab:violation-draft}
\end{table}

%\newpage

\vspace*{-0.8cm}

\section{Results}




% \begin{table}[h!]
% \centering
% \scriptsize
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|}
% \hline
% \rowcolor[HTML]{333333} 
% {\color[HTML]{FFFFFF} \textbf{quic\_client\_test\_prefadd\_error}} \\
% \begin{tabular}[c]{@{}l@{}}Zero length CID for preferred\_address transport parameter. Must have TRANS\\ PORT\_PARAMETER\_ERROR.\end{tabular} \\ \hline
% \end{tabular}
% }
% \caption{Transport parameter errors }
% \label{tab:tp-error}
% \end{table}


%\vspace*{-0.6cm}

%\clearpage


%\todo{localhost, monde parfait}
We run 100 iterations of each test on each implementation. This is to allow diverse behaviour to be captured and evaluated by the tool. Remember that each iteration generates different packets traces following the random generation approach described above. Each test was run in localhost, thus we can assume a perfect link. The results obtained against \texttt{QUIC} servers are briefly presented in Table \ref{tab:server-glob}. Those for \texttt{QUIC} clients are given in Table \ref{tab:client-glob}.  There, each column contains the results for a specific \texttt{QUIC} implementation. Each row contains the results of a test. The success rate in each cell represents the percentage of test runs satisfying all the specification requirements.

Observe that the interpretation of statistical models based on our results could be biased by the distribution of some errors.
Indeed, a few requirements could be violated for a large number of test iterations. This would lead the test to have a very low success rate while the implementation could meet all the other requirements checked by this test. For example, the \texttt{picoquic} implementation does not support migration properly. It lowers the success rate of the \texttt{stream} test to around 50\% while in practice, only one requirement is violated.

In fact, those success rates depict an insight of the implementations maturity.
This shall not be seen as a problem, as our objective is to detect errors in implementations rather than reasoning statistically.
Indeed, the detailed results express the requirements which are not met. This can give some clues for the debugging.

%A failed test stops when a requirement is not respected.
%An example of such problem is with the  "\texttt{unknown}" test that verifies the requirements linked to unknown frames. It is part of the tests we implemented.  The test is successful if the tested implementation sends a \texttt{FRAME\_ENCODING\_ERROR} upon receiving this unknown frame. The test is considered as failed when the error is not received.
%By exploiting the random generation approach, test run generation should give rise to the two events\todo{two ?}.
%In Table \ref{tab:server-glob}, we observe that most implementations managed to return the correct transport error code. However, implementation error code\todo{ici c'est erreur de codage} may happen. As an example, the implementation \texttt{quant} stops its execution and does not report any error while the implementation \texttt{aioquic} reports an incorrect error code and sometimes crashes.  Only looking at the number of tests passed for \texttt{aioquic} or \texttt{quant} could lead to the conclusion that they have a lot of faults. However, our analysis suggests that most of the errors are linked to the migration and removing this process increases a lot the success rate of both implementation.


% changes the weight of the frame distribution and
%properties
%A new test verify the properties linked to an "\texttt{unknown}" frame. It was not possible to generate this frame before.

%Another example is with the \texttt{picoquic} implementation and the \texttt{quic\_server\_test\_stream} given in Section \ref{server_impl_test}, only inspecting the value in the cells could indicate that \texttt{picoquic} does not respect the specifications but when we check the details we notice that only one requirement frequently fail.



%\vspace*{-0.3cm}

\begin{table}%[H]
\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\setlength\tabcolsep{2pt}
\begin{tabular}{|l|ccccccc|}
\hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{quinn} \cite{quinn}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{mvfst} \cite{mvfst}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{picoquic} \cite{picoquic}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{quic-go} \cite{quic-go}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{aioquic} \cite{aioquic}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{quant} \cite{quant}}} &
  \rotatebox{90}{\textbf{quiche}  \cite{quiche}} \\ \hline
\textbf{stream} &
  % \cellcolor[HTML]{32CB00}100\% & % no migration
  \cellcolor[HTML]{00ff55} 79\%  & 
  
\cellcolor[HTML]{FE0000} 6\%  & 
\cellcolor[HTML]{ffbb33} 56\%  &  
\cellcolor[HTML]{009933} 95\%  & 
\cellcolor[HTML]{ff6666} 18\%  & 
\cellcolor[HTML]{ff6666} 12\%  & 
  \cellcolor[HTML]{009933}97\% \\ \cline{1-1}
\textbf{max} &
  %\cellcolor[HTML]{009933}97\% &
  \cellcolor[HTML]{009933} 85\%  & 
  
\cellcolor[HTML]{FE0000} 3\%  & 
\cellcolor[HTML]{ffbb33} 47\%  & 
\cellcolor[HTML]{e69900} 39\%  & 
\cellcolor[HTML]{e69900} 27\%  & 
\cellcolor[HTML]{ff6666} 21\%  &
  \cellcolor[HTML]{009933}96\% \\ \cline{1-1}
\textbf{reset\_stream} &
  %\cellcolor[HTML]{F8A102}34\% &
  \cellcolor[HTML]{e69900} 29\%  & 
  
\cellcolor[HTML]{FE0000} 7\%  & 
\cellcolor[HTML]{ffff00} 61\%  & 
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{ff6666} 24\%  & 
\cellcolor[HTML]{FE0000} 5\%  & 
  \cellcolor[HTML]{009933}98\% \\ \cline{1-1}
\textbf{connection\_close} &
  %\cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933} 95\%  &
  
\cellcolor[HTML]{e69900} 37\%  & 
\cellcolor[HTML]{00ff55} 81\%  & 
\cellcolor[HTML]{ffff00} 63\%  & 
\cellcolor[HTML]{00ff55} 78\%  & 
\cellcolor[HTML]{e69900} 40\%  & 
  \cellcolor[HTML]{009933}100\% \\ \cline{1-1}
\textbf{stop\_sending} &
  %\cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}100\% &
  
\cellcolor[HTML]{FE0000} 4\%  & 
\cellcolor[HTML]{ffbb33} 48\%  & 
  \cellcolor[HTML]{F8A102}33\% &
\cellcolor[HTML]{e69900} 33\%  & 
\cellcolor[HTML]{FE0000} 8\%  & 
  \cellcolor[HTML]{009933}96\% \\ \cline{1-1}
\textbf{accept\_maxdata} &
  %\cellcolor[HTML]{34FF34}91\% &
  \cellcolor[HTML]{00ff55} 77\%  & 
  
\cellcolor[HTML]{ff6666} 12\%  & 
\cellcolor[HTML]{ffbb33} 50\%  & 
\cellcolor[HTML]{ffff00} 68\%  & 
\cellcolor[HTML]{ffbb33} 43\%  & 
\cellcolor[HTML]{ff6666} 21\%  & 
  \cellcolor[HTML]{009933}96\% \\ \cline{1-1}
% \textbf{ext\_min\_ack\_delay} &
%   %\cellcolor[HTML]{34FF34}78\% &
%   \cellcolor[HTML]{00ff55} 80\%  & 
  
% \cellcolor[HTML]{FE0000} 10\%  & 
% \cellcolor[HTML]{e69900} 38\%  & 
% \cellcolor[HTML]{009933} 100\%  & 
% \cellcolor[HTML]{e69900} 26\%  & 
% \cellcolor[HTML]{FE0000} 6\%  & 
%   \cellcolor[HTML]{009933}98\% \\ \cline{1-1}
  \textbf{unknown} &
  \cellcolor[HTML]{009933}95\% &
  \cellcolor[HTML]{009933}99\% &
  \cellcolor[HTML]{009933}99\% &
  \cellcolor[HTML]{009933}96\% &
  \cellcolor[HTML]{FE0000}{0\%} &
  \cellcolor[HTML]{FE0000}{0\%} &
  \cellcolor[HTML]{009933}100\% \\ \cline{1-1}
\textbf{unkown\_tp} &
\cellcolor[HTML]{00ff55} 84\%  & 
\cellcolor[HTML]{ffbb33} 59\%  & 
\cellcolor[HTML]{009933} 98\%  & 
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{ffff00} 68\%  & 
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{009933} 96\%  \\  \cline{1-1}
\textbf{double\_tp\_err} &
  \cellcolor[HTML]{FE0000}{0\%} &
  %\cellcolor[HTML]{FFCB2F}65\% &
  \cellcolor[HTML]{FE0000} 0\%  & 
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{FE0000}{0\%} &
  \cellcolor[HTML]{FE0000}3\% &
  \cellcolor[HTML]{009933}100\% \\ \cline{1-1}
\textbf{tp\_err} &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{FE0000}0\% \\ \cline{1-1}
\textbf{tp\_acticoid\_err} &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{FE0000}0\% \\ \cline{1-1}
\textbf{no\_icid\_err} &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{FE0000}0\% \\ \cline{1-1}
  \textbf{token\_err} &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}98\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}{\color[HTML]{333333} 100\%} &
  \cellcolor[HTML]{009933}{\color[HTML]{333333} 100\%} &
  \cellcolor[HTML]{009933}99\% \\ \cline{1-1}
% new\_token\_err &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l|}{} \\ \cline{1-1}
\textbf{new\_token\_err} & 
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{00ff55} 84\%  & 
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  \\ \cline{1-1}
\textbf{handshake\_done\_err} &
  \cellcolor[HTML]{009933}100\% &
  \cellcolor[HTML]{009933}92\% &
  \cellcolor[HTML]{009933}89\% &
  \cellcolor[HTML]{FE0000}0\% &
  \cellcolor[HTML]{009933}86\% &
  \cellcolor[HTML]{FE0000}2\% &
  \cellcolor[HTML]{00ff55}77\% \\ \cline{1-1}
 
% newconnectionid\_err &
%   &
%   &
%   &
%   &
%   &
%   &
%   \\ \cline{1-1}
\textbf{newcid\_err} & 
\cellcolor[HTML]{00ff55} 81\% & 
\cellcolor[HTML]{009933} 85\%  & 
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{FE0000} 9\%  & 
\cellcolor[HTML]{ffff00} 68\%  & 
\cellcolor[HTML]{009933} 93\%  & 
\cellcolor[HTML]{009933} 91\% \\ \cline{1-1}
% max\_limit\_err &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l|}{} \\ \hline
\textbf{max\_limit\_err} & 
\cellcolor[HTML]{ffbb33} 49\%  & 
\cellcolor[HTML]{ffbb33} 41\%  & 
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{ffbb33} 41\%  & 
\cellcolor[HTML]{ff6666} 16\%  & 
\cellcolor[HTML]{FE0000} 0\%   \\ \cline{1-1}

\textbf{blocked\_err} &
  \multicolumn{1}{c}{\cellcolor[HTML]{34FF34}70\%} &
  \multicolumn{1}{c}{\cellcolor[HTML]{FE0000}0\%} &
  \multicolumn{1}{c}{\cellcolor[HTML]{FE0000}0\%} &
  \multicolumn{1}{c}{\cellcolor[HTML]{34FF34}75\%} &
  \multicolumn{1}{c}{\cellcolor[HTML]{FE0000}{0\%}} &
  \multicolumn{1}{c}{\cellcolor[HTML]{FE0000}{0\%}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{009933}100\%} \\ \cline{1-1}
% retirecoid\_err &
%   \multicolumn{1}{c}{\cellcolor[HTML]{32CB00}100\%} &
%   \multicolumn{1}{c}{\cellcolor[HTML]{FE0000}0\%} &
%   \multicolumn{1}{c}{\cellcolor[HTML]{32CB00}100\%} &
%   \multicolumn{1}{c}{\cellcolor[HTML]{FE0000} ? } &
%   \multicolumn{1}{c}{\cellcolor[HTML]{FE0000}{0\%}} &
%   \multicolumn{1}{c}{\cellcolor[HTML]{FE0000}{0\%}} &
%   \multicolumn{1}{c|}{\cellcolor[HTML]{FE0000}0\%} \\ \cline{1-1}
\textbf{retirecid\_err} & 
\cellcolor[HTML]{009933} 87\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{009933} 86\%  & 
\cellcolor[HTML]{009933} 85\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  \\ \cline{1-1}
\textbf{stream\_limit\_err} &
\cellcolor[HTML]{009933} 100\% &
\cellcolor[HTML]{ffbb33} 63\% &
\cellcolor[HTML]{009933} 99\%  & 
\cellcolor[HTML]{009933} 98\%  & 
\cellcolor[HTML]{009933} 99\%  & 
\cellcolor[HTML]{FE0000} 10\%  & 
\cellcolor[HTML]{FE0000} 0\%  \\ \cline{1-1}
% crypto\_limit\_err &
%   &
%   &
%   &
%   &
%   &
%   &
%   \\ \cline{1-1}
\textbf{newcid\_length\_err} &
\cellcolor[HTML]{00ff55} 84\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 2\%  & 
\cellcolor[HTML]{00ff55} 81\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{009933} 91\%  \\ \cline{1-1}
\textbf{newcid\_rtp\_err} & 
\cellcolor[HTML]{009933} 91\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{009933} 90\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  \\ \cline{1-1}
% max\_err &
%   &
%   &
%   &
%   &
%   &
%   &
%   \\ \hline
\textbf{max\_err} & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{009933} 90\% &
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  \\ \hline
\end{tabular}%
}
\caption{Server - Successful test ratio}
\label{tab:server-glob}
%\vspace{-2em}
\vspace*{-0.9cm}
\end{table}



%\clearpage


%\subsection{Client implementations}

% An example is the  "\texttt{unknown}" test that verifies the properties linked to unknown frames. It is part of the tests we implemented. 
% %A new test verify the properties linked to an "\texttt{unknown}" frame. It was not possible to generate this frame before. 
% The test is successful if the tested implementation sends a \texttt{FRAME\-\_ENCODING\-\_ERROR} upon receiving this unknown frame. The test is considered as failed when the error is not received over its course. 
% %If we don't receive this error when we send this frame, the test is failed. 
% %To allow the generation of unknown frame at any time in 1-RTT encryption level, we set an high relative weight to it to influence its distribution.
% The test changes the weight of the frame distribution 
% %\newpage
% during the packets generation to make such a frame appear. In Table \ref{tab:server-glob}, we observe that most implementations managed to return the correct error code. However, different erroneous behaviour has been observed. For instance, \texttt{quant} stops its execution and does not report any error while \texttt{aioquic} reports an incorrect error code and sometimes crashes.

%\noindent 

%\newpage

\begin{table} %[H]
\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\setlength\tabcolsep{2pt}
\begin{tabular}{|l|ccccccc|}
\hline
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{quinn} \cite{quinn}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{picoquic} \cite{picoquic}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{quic-go} \cite{quic-go}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{aioquic} \cite{aioquic}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{quant} \cite{quant}}} &
  \multicolumn{1}{c|}{\rotatebox{90}{\textbf{quiche} \cite{quiche}}} &
  \rotatebox{90}{\textbf{lsquic}  \cite{lsquic}} \\ \hline
\textbf{stream} &
  \cellcolor[HTML]{009933} 99\% &
  \cellcolor[HTML]{ffbb33} 51\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{009933} 97\% &
  \cellcolor[HTML]{00ff55} 85\% &
  \cellcolor[HTML]{ffbb33} 52\% &
  \cellcolor[HTML]{009933} 92\% \\ \cline{1-1}
\textbf{max} &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{ff6666} 15\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{009933} 98\% &
  \cellcolor[HTML]{00ff55} 85\% &
  \cellcolor[HTML]{e69900} 34\% &
  \cellcolor[HTML]{009933} 100\% \\ \cline{1-1}
\textbf{accept\_maxdata} &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{009933} 93\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{009933} 97\% &
  \cellcolor[HTML]{009933} 95\% &
  \cellcolor[HTML]{00ff55} 82\% &
  \cellcolor[HTML]{00ff55} 83\% \\ \cline{1-1}
% ext\_min\_ack\_delay &
%   \cellcolor[HTML]{009933} 100\% &
%   \cellcolor[HTML]{e69900} 40\% &
%   \cellcolor[HTML]{009933} 99\% &
%   \cellcolor[HTML]{009933} 100\% &
%   \cellcolor[HTML]{009933} 100\% &
%   \cellcolor[HTML]{009933} 100\% &
%   \cellcolor[HTML]{009933} 95\% \\ \cline{1-1}
\textbf{unkown} &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{009933} 96\% &
  \cellcolor[HTML]{009933} 99\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{FE0000} 0\% \\ \cline{1-1}
\textbf{tp\_unkown} &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{e69900} 34\% &
  \cellcolor[HTML]{009933} 99\% &
  \cellcolor[HTML]{009933} 99\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{009933} 99\% &
  \cellcolor[HTML]{009933} 96\% \\ \cline{1-1}
\textbf{double\_tp\_error} &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% \\ \cline{1-1}
\textbf{tp\_error} &
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{009933} 100\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\%  & 
\cellcolor[HTML]{FE0000} 0\% \\ \cline{1-1}
\textbf{tp\_acticoid\_error} &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% \\ \cline{1-1}
\textbf{no\_ocid} &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% \\ \cline{1-1}
\textbf{tp\_prefadd\_error} &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% \\ \cline{1-1}
\textbf{blocked\_error} &
  \cellcolor[HTML]{009933} 99\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{009933} 97\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{009933} 91\% &
  \cellcolor[HTML]{009933} 98\% \\ \cline{1-1}
\textbf{retirecoid\_error} &
  \cellcolor[HTML]{009933} 99\% &
  \cellcolor[HTML]{009933} 99\% &
  \cellcolor[HTML]{009933} 100\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{009933} 98\% \\ \cline{1-1}
\textbf{new\_token\_error} &
  \cellcolor[HTML]{009933} 98\% &
  \cellcolor[HTML]{009933} 94\% &
  \cellcolor[HTML]{009933} 96\% &
  \cellcolor[HTML]{FE0000} 1\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{00ff55} 87\% &
  \cellcolor[HTML]{009933} 100\% \\ \cline{1-1}
% handshake\_done\_error &
% \cellcolor[HTML]{FE0000} 3\%  & 
% \cellcolor[HTML]{00ff55} 85\%  & 
% \cellcolor[HTML]{FE0000} 0\%  & 
% \cellcolor[HTML]{ffff00} 69\%  & 
% \cellcolor[HTML]{FE0000} 4\%  & 
% \cellcolor[HTML]{ffff00} 69\%  & 
% \cellcolor[HTML]{FE0000} 0\%\\ \cline{1-1}
\textbf{limit\_max\_error} &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{00ff55} 88\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{00ff55} 81\% &
  \cellcolor[HTML]{FE0000} 0\% &
  \cellcolor[HTML]{FE0000} 0\% \\ \hline
\end{tabular}%
}
\caption{Client - Successful test ratio}
\label{tab:client-glob}
%\vspace{-2em}
\vspace*{-1cm}
\end{table}

%\todo{uniformise "packet and frame"}

%However, even if not all information can be found in these tables, we can still have an overview of the results.\todo{on met ?}

We will now present the two main categories of problems found. The first one concerns all problems related to migration and the second one concerns those related to the transport errors. Note that due to the page limitation, we did not include all the results but these will be available in a technical version of the paper.

%\todo{rajouter des subsection}
\subsection{Migration issues}

%We first want to mention that we were unable to properly test all implementations.
%We first want to mention that all implementations were not always testable in all cases because of \texttt{TLS} problems. As an example, it is the case for the server test with \texttt{lsquic} where we get a \texttt{TLS} internal error. It is also the case with the client for \texttt{mvfst} where the decryption was problematic, we believe that this is due to zero-length source connection ID which is not currently supported. The reason behind this is that all features of \texttt{QUIC} and \texttt{TLS} are not implemented in our formal specification of \texttt{QUIC}. However, we managed to improve the compatibility between \texttt{Ivy} and other implementations. This problem is also present for other testing tools used for \texttt{QUIC} \cite{Piraux_2018}.

For the tests with only legal frames/packets, we do not detect many different errors. Most of the problems are linked to acknowledgement of acknowledgements and the path validation during a migration. 

The first problem never leads to a crash and no major security issues were detected. We supposed that it is also linked to migration since this error amplifies when migration is allowed. This is enhanced when we compare the result of the client tests and the server tests. This error is less present when the client is tested. As a reminder, the server tests allow multiple connection migrations while and client tests disable it.

However the migration problems are more serious. Many security considerations are involved in guaranteeing authentication, confidentiality and integrity of the messages exchanged between endpoints with the migration in general. Many attacks are linked to the migration such as
the "Peer Address Spoofing", "On-Path Address Spoofing" or the "Off-Path Packet
Forwarding" describe in the \texttt{QUIC} specification. It is important for the path and
address validation to be well implemented.




\vspace*{-0.1cm}
\subsubsection{Migration issues: Case study I}
\hfill\\

\vspace*{-0.3cm}
An example of problem with the migration was highlighted with \texttt{mvfst} implementation. The migration is considered invalid when we start it just after receiving the \texttt{HANDSHAKE\_DONE} and the \texttt{disable\_active\_migration} transport parameter is not set according to Wireshark and our tool. In this case we acknowledge the frame in the migrated connection. According to Section 9 of the specifications, an endpoint cannot migrate before the handshake is confirmed. From the client point of view, we consider the handshake as confirmed when we received the \texttt{HANDSHAKE\_DONE} frame.

For the server, the handshake is confirmed when the handshake is complete. It happens when the \texttt{TLS} stacks had both sent a "Finished" message and verified the peer’s "Finished" message. 

Thus, if a client migrates just after it receives a \texttt{HANDSHAKE\-\_DONE}, then the client respects the draft. The server has to accept the migration before it receives the \texttt{ACK} for the \texttt{HANDSHAKE\_DONE}. 

However the \texttt{mvfst} implementation server only knows that the client considers the handshake as confirmed when it received the \texttt{ACK} for \texttt{HANDSHAKE\_DONE}. We suppose that \texttt{mvfst} wants to be sure that the client has received the \texttt{HANDSHAKE\_DONE} before allowing it to migrate.  Moreover, in the case where the frame is acknowledged in the original connection, this problem does not arise. This is consistent with our hypothesis. %A deeper source code analysis or questions to the developers should be introduced to get a full answer.

%\todo{parler que c'est good dans l'autre cas}

% With a source code analysis, we know that the problem is from the \texttt{ServerStateMachine.cpp} file of \texttt{mvfst} repository and the \texttt{disableMigration} setting for the transport connection is set to true even if the \texttt{disable\_}- \texttt{active\_migration} transport parameter was not send by both endpoints\todo{remove ?}.

\subsubsection{Migration issues: Case study II}
\hfill\\
% It can also be ambiguous.
%because we are not sure when we are allowed to perform migration which makes fail the connection $50$\%.\todo{explain}



Another problem reflected in our model is that polysemous requirements in the draft lead to different valid formal interpretations. This means that they are ambiguous. The best example is with the
highest-numbered non-probing packet to which an endpoint should send its packets. Consider the following statement:

%\resizebox{\columnwidth}{!}{%
\vspace*{-0.1cm}


\epigraph{ "\textit{An endpoint only changes the address that it sends packets to in\\
response to the highest-numbered non-probing packet.  This ensu-\\
res that an endpoint does not send packets to an old peer address\\in the case that it receives reordered packets}."}{Draft 29 of \texttt{QUIC} section 9.3.}
%}
\vspace*{-0.1cm}


According to this rule, we should send the packet to the highest-numbered non-probing packet. A non-probing packet is a packet containing any other frame than the probing frames which are \texttt{PATH\_CHALLENGE}, \texttt{PATH\_RESPONSE}, \texttt{NEW\_CO}- \texttt{NNECTION\_ID}, and \texttt{PADDING} frames.  As we did not have an indication about the encryption level to consider, we used the highest-numbered non-probing packet among all possible ones. Since migration is allowed only after the handshake completed, we should probably consider only the encryption level for the 0-RTT Protected or short header packets. It is not written explicitly.

However, in the same paragraph, we can find the following indication:

\vspace*{-0.1cm}

\epigraph{ "\textit{Receiving a packet from a new peer address containing a non-probing frame
indicates that the peer has migrated to that address. In response to such a packet, an
endpoint MUST start sending subsequent packets to the new peer address and MUST
initiate path validation (Section 8.2) to verify the peer’s ownership of the
unvalidated address}."}{Draft 29 of \texttt{QUIC} section 9.3.}

\vspace*{-0.1cm}

%\clearpage

\noindent
If we use this rule, then we must send responses of non-probing frames to the new peer address. When we consider the highest-numbered non-probing packet among all the possible encryption level, most of the implementation do not pass the requirement. This is the case with \texttt{picoquic}. However when we consider the highest-numbered non-probing packet among the application encryption level, some of the implementations that do not pass with the above interpretation manage to pass the requirement. This is again the case for \texttt{picoquic}. We show that both chosen interpretations of the requirement, which are valid from a formal point of view, lead to different results. Even if the best solution seems trivial for a network specialist, the ambiguity should be removed.

%Now, the question is the following: why do these rules, in the same paragraph, seem to contradict one another when we consider them in pairs ? What should we do if the highest-numbered non-probing packet is received on the old peer address ? Is it the highest among all packets or among application packets ? Even if this question seems trivial for a network specialist, the ambiguity should be removed. \todo{rethorique}

\vspace*{-0.1cm}
\subsection{Transport error code issues}

\vspace{-0.1cm}

Concerning the management of the transport error code, we can see that some implementations respect the specification better than others. Various types of errors have been observed. We faced some implementations that do not implement a requirement in the specification. For example, the transport error codes management is almost completely implemented in some implementations (e.g \texttt{quinn}) and barely implemented in other ones (e.g. \texttt{quant}) as can see in Table \ref{tab:server-glob}. As the application layer can use those error codes to decide whether to fall back on a \texttt{TCP} connection, the transport error codes management is important. 

%\todo{more advanced ne veut rien dire. A corriger avec Tom}

Another type of problem is when implementations use the wrong encryption level. This is mostly the case for \texttt{aioquic} or \texttt{quinn}. Those two implementations use the \texttt{1-RTT} encryption scheme to return the error. However this encryption level is not allowed at this time. 

Some implementations do not check if a specific frame is allowed by their peers. For example, the \texttt{NEW\_TOKEN} frame (sent by \texttt{picoquic} and \texttt{mvfst}) is not allowed to be sent by the client. These implementations do not report any \texttt{PROTOCOL\_VIOLATION} that does not conform to the specification, neither local error. %\todo{Discuter et réécrire cette phrase: peers n'est pas défini et la conclusion est vague}.




%Our tests stop each time we find a situation where a requirement is not respected. It is considered as failed. If every requirement is respected and that the test ends, it is a success. We decide to launch the same test for 100 iterations for each implementation in order to find a maximum of erroneous behaviour. This number is defined by time constraint.



%\todo{(mp): Il manque une description générale des conclusions de la table}

%The results we obtained highlight several types of errors.
%The most important part of this work is the type of errors found. 
%Some of them are non-implemented features. Others are violations of the specification or result from ambiguities in the draft. We can observe an ambiguity when encountering different behaviours adopted by implementations for a given requirement. 
%These choices can lead to unwanted behaviour from the tested implementation.\todo{(mp): pas clair c'st linked a la phrase d'avant en fait mais on avait l'example de mvfst ou la migration de se finissait jamais car on sait pas clairement quand l'autre a complete le handshake => donc unwanted dans le sens ou on arrive pas a faire la migr   ation} 
%We also found concurrency errors. <-- \todo{(mp): Donnez un exemple court et parlant, c'est quoi une concurrency error ?  les threads "paniquing" (un message erreur rust) puis ca crash}
%On peut juste dire que l'implémentation a eu un crash non ?
%On peut nommer ça plus généralement "programming error"
%Our tool exposed programming errors and crashes in some implementations.
%One implementation also produce a concurrency error with the managemnt of \texttt{NEW\_CONNECTION\_ID} frame
%The results we obtained demonstrate that most implementations are affected by an ambiguity regarding the \texttt{QUIC} migration. %Many problems linked to the migration of client were observed.

%Finally, we manage to test one \texttt{QUIC} transport extension but no significant errors were found since some very important properties are impossible to verify with Ivy. However this shows that the methodology proposed by McMillan and Zuck can be used to verify \texttt{QUIC} transport extension in a practical manner. 



 
%But it also happens that the implementation occasionally locally crash.

%Our experiments clearly show that some implementations are more advanced than others for some feature of QUIC. Some tests are passed by most of the implementations while others have a low success rate. This perception is well reflected when we compare the result of the client and the server tests. As a reminder, with the server tests multiple connection migration are allowed in server tests and disabled in client tests.\todo{on met avant?} %Only looking at the number of tests passed for \texttt{aioquic} or \texttt{quant} could lead to the conclusion that they have a lot of faults. However, our analysis suggests that most of the errors are linked to the migration and removing this process increases a lot the success rate of both implementation.
%However, one should focus on the type of error rather than the number of errors since it could be misinterpreted or lead to a false conclusion on the quality of the implementation

We also observed that some implementation send error codes with the wrong error message. As an example, when we send \texttt{HANDSHAKE\_DONE} frame to the \texttt{quic-go} server, which is not allowed, it closes the connection with the message error reporting that this frame is not allowed because of the encryption level. This is not correct in this case. 


%\todo{citer les implem}

%The transport error codes management also underlines that some implementations are violating the specification of the draft. 
Some implementations return the wrong error code. An example is \texttt{mvfst} when we send \texttt{NEW\_CONNECTION\_ID} frame with an invalid field, \texttt{mvfst} detects the correct problem but return the wrong error code. We know it detects the problem since the error message describe the fact that the field is invalid.

%Other implementations return an error which does not correspond to the current problem. An example is given with\texttt{quic-go} when our test tool send \texttt{HANDSHAKE\_DONE} frame as clients which is not allowed. It reports that the frame is not allowed at the current encryption level instead of reporting that the endpoint cannot send this frame at all.

Some implementations like \texttt{quant} detect the error locally without reporting an error. This is not conforming to the specification. However, when we analyse the latest version, that problem has been solved as presented in Table \ref{tab:quant}.

%\newpage

\vspace*{-0.3cm}

%\newpage

\begin{table}[H]
\centering
\small
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cc|}
\hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{FFFFFF}}} &
  \multicolumn{1}{c|}{\textbf{quant \textit{29}}} &
 \textbf{quant \textit{master}} \\ \hline
\textbf{double\_tp\_error} &
  \cellcolor[HTML]{FE0000}3\% &
  \cellcolor[HTML]{009933}100\% \\ \cline{1-1}
\textbf{tp\_error} &
  \cellcolor[HTML]{FE0000}0\% &
\cellcolor[HTML]{009933} 100\%   \\ \cline{1-1}
\textbf{tp\_acticoid\_error} &
  \cellcolor[HTML]{009933}100\% &
\cellcolor[HTML]{009933} 100\%  \\ \cline{1-1}
\textbf{no\_icid\_error } &
  \cellcolor[HTML]{FE0000}0\% &
\cellcolor[HTML]{009933} 100\% \\ \hline
\end{tabular}%
%}
\caption{Quant transport parameter: before/after}
\vspace*{-0.5cm}
\label{tab:quant}
\end{table}

%This example shows how Ivy can be used to track the evolution of an implementation. We also found errors for \texttt{aioquic} and managed to fix them. \todo{ok ?}

%\vspace*{-1.5cm}

% Sommet page 2
% Presenter 1 test

%\vspace{10cm}

%\section*{Conclusion}



% sommaire contribution
% type de bug etc
% presenter en detail dans poster

%\section{Future Work}

\section*{Conclusion and Future Work}

%\todo{+++diversite resultat => ambiguité => prouve que ca fonctionne}

In this paper, we applied the Ivy modelization framework to \texttt{QUIC} and produced a model verifying a large part of the requirements of the \texttt{QUIC} specification. The model contains new and updated requirements from the original work. We automated the use of the model in a series of tests against \texttt{QUIC} clients and servers. We showed the diversity of results we obtained with our tool and the variety of errors encountered. In addition, the results we obtained illustrate the ability of the tool to highlight ambiguities in the specification and generate executions following different interpretations of these ambiguities. This shall be exploited to improve the IETF specification of \texttt{QUIC}.

%In this short paper, we demonstrate how to apply the Ivy modelization framework to verify the requirements of the \texttt{QUIC} specification on its implementations. We 

%In particular, while they limited themselves to four implementations of \texttt{draft-18}, we have been able to consider seven implementations, of both the server and the client, of  \texttt{draft-29}. Moreover, we managed to consider the validation of many rules that they could not verify in their previous work. We observed that, albeit Ivy is not well suited to model all requirements of the protocol, the approach can be used to identify a considerable number of errors in those implementations. Besides, it can be used to highlight ambiguities in the specification. As presented before, we show that according to the chosen interpretation of an ambiguous requirement, all valid from a formal point of view, we observe the corresponding diversity in the results. This shall be exploited to improve the IETF specification of \texttt{QUIC}.

We see several directions for future work. One of them is to include in our approach extensions and additional features of \texttt{QUIC} such as \texttt{Multipath QUIC}~\cite{10.1145/3143361.3143370}, \texttt{Forward Erasure Correction} (FEC)~\cite{michel2019quic}, the Unreliable Datagram extension \cite{pauly2018unreliable} and packets such as \texttt{Retry} and \texttt{Version Negotiation}.

%Completing Ivy with the missing packets should also be done. Examples of such packets
%are the \texttt{Retry} and \texttt{Version Negotiation}. It is possible to add them in the current model of Ivy. 

\vspace*{-0.2cm}

\section*{Software artefacts}

We will release our modifications to Ivy, the updated test suite and the Docker images automating the tests~\cite{TowardsverificationofQUICextensions}\footnote{\url{https://github.com/AnonyQUIC/QUIC-Ivy}}. Here are the commits of the tested implementations:

\vspace*{-0.3cm}

\begin{table}[H]
\centering
\small

\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\textbf{picoquic (C)}  \cite{picoquic} & \textbf{lsquic}         \cite{lsquic}           \\
ad23e6c3593bd987dcd8d74fc9f528f2676fedf4   & v2.29.4                                      \\ \cline{2-2} 
\textbf{picotls}  \cite{picotls}               & \textbf{boringssl}           \cite{boringssl}      \\
47327f8d032f6bc2093a15c32e666ab6384ecca2 & a2278d4d2cabe73f6663e3299ea7808edfa306b9 \\ \hline
\textbf{quic-go (golang)}    \cite{quic-go}    & \textbf{quinn (rust)}     \cite{quinn}         \\
v0.20.0                                    & 0.7.0                                        \\ \hline
\textbf{aioquic (python)}   \cite{aioquic}     & \textbf{quiche (rust)}     \cite{quiche}        \\
0.9.3                                      & 0.7.0                                        \\ \hline
\textbf{quant (C)}    \cite{quant}           & \textbf{mvfst (facebook/C++)}     \cite{mvfst} \\
29                                         & 36111c1                                      \\ \hline
\end{tabular}%
}
\caption{Draft 29 tested implementations}
\label{tab:QUIC-Implementations}
\end{table}





% Cite rfc 9000, McMillan paper, Papier Ivy


%(mp): Oui, mais on ne sait pas quand, et probablement lors d'une autre publication donc on peut l'enlever.

%\section{ACKNOWLEDGEMENT}







==> garbage.tex <==
%\subsection{Why formal verification ?}
%\todo{needed since present in the introduction ?}
%The most common way to test if an implementation of a protocol has the properties that we %expect is to operate it with other implementations. We check if it has the expected behaviour. %H%owever, experience has shown that this approach suffers from several drawbacks. First, if an %inconsistency of the specification is noticed between the two implementations, the errors will %be corrected in the implementations themselves. There is no clear view of what an %implementation should do to fit the specification. The test coverage is also low because most %implementations do not implement all the properties allowed by the standard. The last reason %is also that you cannot do interoperability with an implementation that will be present in the %future. It could completely respect the standards but be impossible to operate with it.

%However formal verification is not perfect either because all properties cannot be verified, %for example we cannot verify properties related to internal state or liveness properties with %this methodology. Multiple valid interpretation for properties can lead to different valid %model which can be problematic but this allow highlighting the potential ambiguity in the %specification. Another important drawback is the computational power needed to run the tests. %Performance should be improved. The last point being that the learning curve is quite big.

%\subsection{Formal verification of QUIC}

% We use the methodology defined by McMillan and Zuck in \cite{}. Our starting point is the QUIC specification [31]. We
% extract all the properties that an implementation should have. We consider all
% the properties as constraints to build a packet. Specific scenarios are created. As
% an example, the goal of a scenario could be to send data or to close a connection.
% The interaction between two implementations can be represented as a graph with
% nodes. To test an implementation, we create a node that is fully respecting the
% specification. We generate the set of all the packets that could be sent by this node
% at time T. We remove from this set all the packets that violate the specification.
% Then, we send one random packet from this set.

% This node is a concrete representation of the protocol. It can send network packets
% that are visible on the wire. We form a system composed of an arbitrary number of
% nodes in which there are at least Ivy, the tested implementation, and the network.
% All nodes from this system have their local specification. All those specifications
% must be respected.

% This methodology is called compositional testing because it composes all the nodes
% together. Each node has an input and an output part. When we compose two
% nodes together, the output of the first node becomes the input of the second one.
% All the assumptions we have from the formal specification on one node are treated
% as a guarantee for its output.


%\texttt{m} We also added \texttt{fuzzing} to transport parameters with the generation and handling of non-standard transport parameters and frames.

%We also implement the QUIC error code module and many corresponding tests that allow to explore a deeper part of the RFC. The previous methodology was extended to allow those tests. We create tests where we voluntary break the specification by generating illegal packets. This is fuzzing and it goes outside the scope of formal verification.

%Finally, the \texttt{min_ack_delay} QUIC extension\cite{iyengar-quic-delayed-ack-02} has also been modelled and is now handled  by Ivy. \todo{dire ca ? Meme si le test donne pas de resultat ouf ?}

%Deployment of the \texttt{QUIC} testing using Ivy has been improved thanks to Docker. It is now more convenient to use and to update. 
% résumer le papier mcmillan avec les résultats clés et l'état des tests dans le papier, bien montrer de quoi on part
% rester vague

% terminer par contribution + presentation du but

% 1 colonne

%\clearpage

Each test generates sequences of different types of frames that respect the specification in order to validate the behaviour of the implementation. We add other similar tests generating other kinds of frames with different distributions. Then we also add a series of tests that verify how implementations behave when they receive undefined frames or undefined transport parameters. Finally, we have a whole category of tests used in order to verify the management of the transport errors by the implementations.%\todo{more explanation needed ? site anonyme avec description?} 

%All tests are detailed in our website\footnote{The URL will be disclosed  \todo{C'est interdit. C'est de l'information cachée. Vous devez soit faire une annexe soit un site web anonymisé} in the camera-ready version}. \todo{C'est 6 pages annexes comprises}

%\todo{explain more != between test}%The tested implementation plays the role of the server and inversely we represent the client.

Note that for the server tests, we allow multiple connection migrations to test its support as well. Several streams are open to test the streams mechanics. We create bidirectional streams. 

%See appendix \ref{test_explanation} for more detailed explanation about the other tests.  
%by increasing the stream ID by four
%to see if the stream management is correct

we One \texttt{QUIC} extension was also verified

We also showed that it was possible to extend McMillan’s work and confirmed that
Ivy was a tool that could be suited for the testing of network protocols. We did not
manage to contact McMillan during our work. Therefore, we refactored the model to make it easier to understand
and extend. This work can be useful for new contributors who want to keep the
update of this formal verification of \texttt{QUIC} extensions in the new specifications. It
is also possible for contributors who will want to use Ivy to test other network
protocols to use our work. As we modelled and tested the properties of one extension,
%we show that there are no limitations for the testing of new \texttt{QUIC} extensions. Moreover, it is quite simple to add new frames, transport parameters and packets to architecture and thus testing extensions.

We can also see the evolution of one implementation according to the draft by
testing different versions. We showed that with quant and observed that most
problems linked to the transport parameters were fixed during the year.

Finally, we showed the usefulness of all our work. By testing eight \texttt{QUIC} implementations
that are, for most of them, at a very advanced stage of development, we
showed that some parts of the specification were not respected. We found different
types of errors.

If you are curious about the full analysis, you can check out \cite{TowardsverificationofQUICextensions}.
